kAgent: An execution-guided crash resolution agent for the Linux kernel

Fuzzing frameworks like syzkaller have uncovered thousands of Linux kernel crashes, many of which are critical and security-sensitive. However, the ability to rapidly repair these crashes has not kept pace, particularly given the complexity and low-level nature of kernel code. Predominantly targeting user-space applications, existing LLM-based program repair techniques are not tailored to the unique challenges posed by kernel fuzz bugs-such as the absence of natural language bug reports, lack of exhaustive test oracles, and highly specialized crash artifacts. Thus, in this work, we first identify the prevalent bottlenecks that generic agents struggle with in complex systems such as the Linux kernel. Guided by these findings, we then build kAgent, a workflow-based agent inspired by how kernel developers diagnose and fix bugs, and kGym++, the co-designed toolstack supporting kAgent's requests. kAgent inspects relevant execution logs, generates execution-grounded natural language hypotheses, synthesizes candidate patches, validates patches through crash reproduction, and iteratively refines its reasoning. We ablate these agentic system features in kAgent and quantitatively analyze their contributions to the overall performance. We also report our experience on building agents for kernel crash repair. Although derived from this work on Linux, we note that our experience applies broadly to fuzzing-discovered bugs in complex systems software. We evaluate kAgent on kBenchSyz and show that it can repair up to 54.5% of crashes without localization and 65% with correct file hints. We also show kAgent's generalization on a few wild Syzkaller bugs, and how different patch types offer varying utility to developers who debug complex system software.

==> icml_template.tex <==
\section{Electronic Submission}

Submission to ICML 2026 will be entirely electronic, via a web site
(not email). Information about the submission process and \LaTeX\ templates
are available on the conference web site at:
\begin{center}
  \texttt{http://icml.cc/}
\end{center}

The guidelines below will be enforced for initial submissions and
camera-ready copies. Here is a brief summary:
\begin{itemize}
  \item Submissions must be in PDF\@.
  \item If your paper has appendices, submit the appendix together with the
        main body and the references \textbf{as a single file}. Reviewers will not
        look for appendices as a separate PDF file. So if you submit such an extra
        file, reviewers will very likely miss it.
  \item Page limit: The main body of the paper has to be fitted to 8 pages,
        excluding references and appendices; the space for the latter two is not
        limited in pages, but the total file size may not exceed 10MB. For the
        final version of the paper, authors can add one extra page to the main
        body.
  \item \textbf{Do not include author information or acknowledgements} in your
        initial submission.
  \item Your paper should be in \textbf{10 point Times font}.
  \item Make sure your PDF file only uses Type-1 fonts.
  \item Place figure captions \emph{under} the figure (and omit titles from
        inside the graphic file itself). Place table captions \emph{over} the
        table.
  \item References must include page numbers whenever possible and be as
        complete as possible. Place multiple citations in chronological order.
  \item Do not alter the style template; in particular, do not compress the
        paper format by reducing the vertical spaces.
  \item Keep your abstract brief and self-contained, one paragraph and roughly
        4--6 sentences. Gross violations will require correction at the
        camera-ready phase. The title should have content words capitalized.
\end{itemize}

\subsection{Submitting Papers}

\textbf{Anonymous Submission:} ICML uses double-blind review: no identifying
author information may appear on the title page or in the paper
itself. \cref{author info} gives further details.

\medskip

Authors must provide their manuscripts in \textbf{PDF} format.
Furthermore, please make sure that files contain only embedded Type-1 fonts
(e.g.,~using the program \texttt{pdffonts} in linux or using
File/DocumentProperties/Fonts in Acrobat). Other fonts (like Type-3)
might come from graphics files imported into the document.

Authors using \textbf{Word} must convert their document to PDF\@. Most
of the latest versions of Word have the facility to do this
automatically. Submissions will not be accepted in Word format or any
format other than PDF\@. Really. We're not joking. Don't send Word.

Those who use \textbf{\LaTeX} should avoid including Type-3 fonts.
Those using \texttt{latex} and \texttt{dvips} may need the following
two commands:

{\footnotesize
\begin{verbatim}
dvips -Ppdf -tletter -G0 -o paper.ps paper.dvi
ps2pdf paper.ps
\end{verbatim}}
It is a zero following the ``-G'', which tells dvips to use
the config.pdf file. Newer \TeX\ distributions don't always need this
option.

Using \texttt{pdflatex} rather than \texttt{latex}, often gives better
results. This program avoids the Type-3 font problem, and supports more
advanced features in the \texttt{microtype} package.

\textbf{Graphics files} should be a reasonable size, and included from
an appropriate format. Use vector formats (.eps/.pdf) for plots,
lossless bitmap formats (.png) for raster graphics with sharp lines, and
jpeg for photo-like images.

The style file uses the \texttt{hyperref} package to make clickable
links in documents. If this causes problems for you, add
\texttt{nohyperref} as one of the options to the \texttt{icml2026}
usepackage statement.

\subsection{Submitting Final Camera-Ready Copy}

The final versions of papers accepted for publication should follow the
same format and naming convention as initial submissions, except that
author information (names and affiliations) should be given. See
\cref{final author} for formatting instructions.

The footnote, ``Preliminary work. Under review by the International
Conference on Machine Learning (ICML). Do not distribute.'' must be
modified to ``\textit{Proceedings of the
  $\mathit{43}^{rd}$ International Conference on Machine Learning},
Seoul, South Korea, PMLR 306, 2026.
Copyright 2026 by the author(s).''

For those using the \textbf{\LaTeX} style file, this change (and others) is
handled automatically by simply changing
$\mathtt{\backslash usepackage\{icml2026\}}$ to
$$\mathtt{\backslash usepackage[accepted]\{icml2026\}}$$
Authors using \textbf{Word} must edit the
footnote on the first page of the document themselves.

Camera-ready copies should have the title of the paper as running head
on each page except the first one. The running title consists of a
single line centered above a horizontal rule which is $1$~point thick.
The running head should be centered, bold and in $9$~point type. The
rule should be $10$~points above the main text. For those using the
\textbf{\LaTeX} style file, the original title is automatically set as running
head using the \texttt{fancyhdr} package which is included in the ICML
2026 style file package. In case that the original title exceeds the
size restrictions, a shorter form can be supplied by using

\verb|\icmltitlerunning{...}|

just before $\mathtt{\backslash begin\{document\}}$.
Authors using \textbf{Word} must edit the header of the document themselves.

\section{Format of the Paper}

All submissions must follow the specified format.

\subsection{Dimensions}

The text of the paper should be formatted in two columns, with an
overall width of 6.75~inches, height of 9.0~inches, and 0.25~inches
between the columns. The left margin should be 0.75~inches and the top
margin 1.0~inch (2.54~cm). The right and bottom margins will depend on
whether you print on US letter or A4 paper, but all final versions
must be produced for US letter size.
Do not write anything on the margins.

The paper body should be set in 10~point type with a vertical spacing
of 11~points. Please use Times typeface throughout the text.

\subsection{Title}

The paper title should be set in 14~point bold type and centered
between two horizontal rules that are 1~point thick, with 1.0~inch
between the top rule and the top edge of the page. Capitalize the
first letter of content words and put the rest of the title in lower
case.
You can use TeX math in the title (we suggest sparingly),
but no custom macros, images, or other TeX commands.
Please make sure that accents, special characters, etc., are entered using
TeX commands and not using non-English characters.

\subsection{Author Information for Submission}
\label{author info}

ICML uses double-blind review, so author information must not appear. If
you are using \LaTeX\/ and the \texttt{icml2026.sty} file, use
\verb+\icmlauthor{...}+ to specify authors and \verb+\icmlaffiliation{...}+
to specify affiliations. (Read the TeX code used to produce this document for
an example usage.) The author information will not be printed unless
\texttt{accepted} is passed as an argument to the style file. Submissions that
include the author information will not be reviewed.

\subsubsection{Self-Citations}

If you are citing published papers for which you are an author, refer
to yourself in the third person. In particular, do not use phrases
that reveal your identity (e.g., ``in previous work \cite{langley00}, we
have shown \ldots'').

Do not anonymize citations in the reference section. The only exception are manuscripts that are
not yet published (e.g., under submission). If you choose to refer to
such unpublished manuscripts \cite{anonymous}, anonymized copies have
to be submitted
as Supplementary Material via OpenReview\@. However, keep in mind that an ICML
paper should be self contained and should contain sufficient detail
for the reviewers to evaluate the work. In particular, reviewers are
not required to look at the Supplementary Material when writing their
review (they are not required to look at more than the first $8$ pages of the submitted document).

\subsubsection{Camera-Ready Author Information}
\label{final author}

If a paper is accepted, a final camera-ready copy must be prepared.
%
For camera-ready papers, author information should start 0.3~inches below the
bottom rule surrounding the title. The authors' names should appear in 10~point
bold type, in a row, separated by white space, and centered. Author names should
not be broken across lines. Unbolded superscripted numbers, starting 1, should
be used to refer to affiliations.

Affiliations should be numbered in the order of appearance. A single footnote
block of text should be used to list all the affiliations. (Academic
affiliations should list Department, University, City, State/Region, Country.
Similarly for industrial affiliations.)

Each distinct affiliations should be listed once. If an author has multiple
affiliations, multiple superscripts should be placed after the name, separated
by thin spaces. If the authors would like to highlight equal contribution by
multiple first authors, those authors should have an asterisk placed after their
name in superscript, and the term ``\textsuperscript{*}Equal contribution"
should be placed in the footnote block ahead of the list of affiliations. A
list of corresponding authors and their emails (in the format Full Name
\textless{}email@domain.com\textgreater{}) can follow the list of affiliations.
Ideally only one or two names should be listed.

A sample file with author names is included in the ICML2026 style file
package. Turn on the \texttt{[accepted]} option to the stylefile to
see the names rendered. All of the guidelines above are implemented
by the \LaTeX\ style file.

\subsection{Abstract}

The paper abstract should begin in the left column, 0.4~inches below the final
address. The heading `Abstract' should be centered, bold, and in 11~point type.
The abstract body should use 10~point type, with a vertical spacing of
11~points, and should be indented 0.25~inches more than normal on left-hand and
right-hand margins. Insert 0.4~inches of blank space after the body. Keep your
abstract brief and self-contained, limiting it to one paragraph and roughly 4--6
sentences. Gross violations will require correction at the camera-ready phase.

\subsection{Partitioning the Text}

You should organize your paper into sections and paragraphs to help readers
place a structure on the material and understand its contributions.

\subsubsection{Sections and Subsections}

Section headings should be numbered, flush left, and set in 11~pt bold type
with the content words capitalized. Leave 0.25~inches of space before the
heading and 0.15~inches after the heading.

Similarly, subsection headings should be numbered, flush left, and set in 10~pt
bold type with the content words capitalized. Leave
0.2~inches of space before the heading and 0.13~inches afterward.

Finally, subsubsection headings should be numbered, flush left, and set in
10~pt small caps with the content words capitalized. Leave
0.18~inches of space before the heading and 0.1~inches after the heading.

Please use no more than three levels of headings.

\subsubsection{Paragraphs and Footnotes}

Within each section or subsection, you should further partition the paper into
paragraphs. Do not indent the first line of a given paragraph, but insert a
blank line between succeeding ones.

You can use footnotes\footnote{Footnotes should be complete sentences.}
to provide readers with additional information about a topic without
interrupting the flow of the paper. Indicate footnotes with a number in the
text where the point is most relevant. Place the footnote in 9~point type at
the bottom of the column in which it appears. Precede the first footnote in a
column with a horizontal rule of 0.8~inches.\footnote{Multiple footnotes can
  appear in each column, in the same order as they appear in the text,
  but spread them across columns and pages if possible.}

\begin{figure}[ht]
  \vskip 0.2in
  \begin{center}
    \centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
    \caption{
      Historical locations and number of accepted papers for International
      Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
      Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this
      figure was produced, the number of accepted papers for ICML 2008 was
      unknown and instead estimated.
    }
    \label{icml-historical}
  \end{center}
\end{figure}

\subsection{Figures}

You may want to include figures in the paper to illustrate your approach and
results. Such artwork should be centered, legible, and separated from the text.
Lines should be dark and at least 0.5~points thick for purposes of
reproduction, and text should not appear on a gray background.

Label all distinct components of each figure. If the figure takes the form of a
graph, then give a name for each axis and include a legend that briefly
describes each curve. Do not include a title inside the figure; instead, the
caption should serve this function.

Number figures sequentially, placing the figure number and caption \emph{after}
the graphics, with at least 0.1~inches of space before the caption and
0.1~inches after it, as in \cref{icml-historical}. The figure caption should be
set in 9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or bottom of a
column, and you may set wide figures across both columns (use the environment
\texttt{figure*} in \LaTeX). Always place two-column figures at the top or
bottom of the page.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require the corresponding stylefiles,
algorithm.sty and algorithmic.sty, which are supplied with this package.
\cref{alg:example} shows an example.

\begin{algorithm}[tb]
  \caption{Bubble Sort}
  \label{alg:example}
  \begin{algorithmic}
    \STATE {\bfseries Input:} data $x_i$, size $m$
    \REPEAT
    \STATE Initialize $noChange = true$.
    \FOR{$i=1$ {\bfseries to} $m-1$}
    \IF{$x_i > x_{i+1}$}
    \STATE Swap $x_i$ and $x_{i+1}$
    \STATE $noChange = false$
    \ENDIF
    \ENDFOR
    \UNTIL{$noChange$ is $true$}
  \end{algorithmic}
\end{algorithm}


\subsection{Tables}

You may also want to include tables that summarize material. Like figures,
these should be centered, legible, and numbered consecutively. However, place
the title \emph{above} the table with at least 0.1~inches of space before the
title and the same after it, as in \cref{sample-table}. The table title should
be set in 9~point type and centered unless it runs two or more lines, in which
case it should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
  \caption{Classification accuracies for naive Bayes and flexible
    Bayes on various data sets.}
  \label{sample-table}
  \begin{center}
    \begin{small}
      \begin{sc}
        \begin{tabular}{lcccr}
          \toprule
          Data set  & Naive         & Flexible      & Better?  \\
          \midrule
          Breast    & 95.9$\pm$ 0.2 & 96.7$\pm$ 0.2 & $\surd$  \\
          Cleveland & 83.3$\pm$ 0.6 & 80.0$\pm$ 0.6 & $\times$ \\
          Glass2    & 61.9$\pm$ 1.4 & 83.8$\pm$ 0.7 & $\surd$  \\
          Credit    & 74.8$\pm$ 0.5 & 78.3$\pm$ 0.6 &          \\
          Horse     & 73.3$\pm$ 0.9 & 69.7$\pm$ 1.0 & $\times$ \\
          Meta      & 67.1$\pm$ 0.6 & 76.5$\pm$ 0.5 & $\surd$  \\
          Pima      & 75.1$\pm$ 0.6 & 73.9$\pm$ 0.5 &          \\
          Vehicle   & 44.9$\pm$ 0.6 & 61.5$\pm$ 0.4 & $\surd$  \\
          \bottomrule
        \end{tabular}
      \end{sc}
    \end{small}
  \end{center}
  \vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost row. Again,
you may float tables to a column's top or bottom, and set wide tables across
both columns. Place two-column tables at the top or bottom of the page.

\subsection{Theorems and Such}
The preferred way is to number definitions, propositions, lemmas, etc.
consecutively, within sections, as shown below.
\begin{definition}
  \label{def:inj}
  A function $f:X \to Y$ is injective if for any $x,y\in X$ different, $f(x)\ne
    f(y)$.
\end{definition}
Using \cref{def:inj} we immediate get the following result:
\begin{proposition}
  If $f$ is injective mapping a set $X$ to another set $Y$,
  the cardinality of $Y$ is at least as large as that of $X$
\end{proposition}
\begin{proof}
  Left as an exercise to the reader.
\end{proof}
\cref{lem:usefullemma} stated next will prove to be useful.
\begin{lemma}
  \label{lem:usefullemma}
  For any $f:X \to Y$ and $g:Y\to Z$ injective functions, $f \circ g$ is
  injective.
\end{lemma}
\begin{theorem}
  \label{thm:bigtheorem}
  If $f:X\to Y$ is bijective, the cardinality of $X$ and $Y$ are the same.
\end{theorem}
An easy corollary of \cref{thm:bigtheorem} is the following:
\begin{corollary}
  If $f:X\to Y$ is bijective,
  the cardinality of $X$ is at least as large as that of $Y$.
\end{corollary}
\begin{assumption}
  The set $X$ is finite.
  \label{ass:xfinite}
\end{assumption}
\begin{remark}
  According to some, it is only the finite case (cf. \cref{ass:xfinite}) that
  is interesting.
\end{remark}
%restatable

\subsection{Citations and References}

Please use APA reference format regardless of your formatter or word processor.
If you rely on the \LaTeX\/ bibliographic facility, use \texttt{natbib.sty} and
\texttt{icml2026.bst} included in the style-file package to obtain this format.

Citations within the text should include the authors' last names and year. If
the authors' names are included in the sentence, place only the year in
parentheses, for example when referencing Arthur Samuel's pioneering work
\yrcite{Samuel59}. Otherwise place the entire reference in parentheses with the
authors and year separated by a comma \cite{Samuel59}. List multiple references
separated by semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
construct only for citations with three or more authors or after listing all
authors to a publication in an earlier reference \cite{MachineLearningI}.

Authors should cite their own work in the third person in the initial version
of their paper submitted for blind review. Please refer to \cref{author info}
for detailed instructions on how to cite your own papers.

Use an unnumbered first-level section heading for the references, and use a
hanging indent style, with the first line of the reference flush against the
left margin and subsequent lines indented by 10 points. The references at the
end of this document give examples for journal articles \cite{Samuel59},
conference publications \cite{langley00}, book chapters \cite{Newell81}, books
\cite{DudaHart2nd}, edited volumes \cite{MachineLearningI}, technical reports
\cite{mitchell80}, and dissertations \cite{kearns89}.

Alphabetize references by the surnames of the first authors, with single author
entries preceding multiple author entries. Order references for the same
authors by year of publication, with the earliest first. Make sure that each
reference includes all relevant information (e.g., page numbers).

Please put some effort into making references complete, presentable, and
consistent, e.g. use the actual current name of authors. If using bibtex,
please protect capital letters of names and abbreviations in titles, for
example, use \{B\}ayesian or \{L\}ipschitz in your .bib file.

\section*{Accessibility}

Authors are kindly asked to make their submissions as accessible as possible
for everyone including people with disabilities and sensory or neurological
differences. Tips of how to achieve this and what to pay attention to will be
provided on the conference website \url{http://icml.cc/}.

\section*{Software and Data}

If a paper is accepted, we strongly encourage the publication of software and
data with the camera-ready version of the paper whenever appropriate. This can
be done by including a URL in the camera-ready copy. However, \textbf{do not}
include URLs that reveal your institution or identity in your submission for
review. Instead, provide an anonymous URL or upload the material as
``Supplementary Material'' into the OpenReview reviewing system. Note that
reviewers are not required to look at this material when writing their review.

% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of the paper
submitted for blind review.

If a paper is accepted, the final camera-ready version can (and usually should)
include acknowledgements.  Such acknowledgements should be placed at the end of
the section, in an unnumbered section that does not count towards the paper
page limit. Typically, this will include thanks to reviewers who gave useful
comments, to colleagues who contributed to the ideas, and to funding agencies
and corporate sponsors that provided financial support.

\section*{Impact Statement}

Authors are \textbf{required} to include a statement of the potential broader
impact of their work, including its ethical aspects and future societal
consequences. This statement should be in an unnumbered section at the end of
the paper (co-located with Acknowledgements -- the two may appear in either
order, but both must be before References), and does not count toward the paper
page limit. In many cases, where the ethical impacts and expected societal
implications are those that are well established when advancing the field of
Machine Learning, substantial discussion is not required, and a simple
statement such as the following will suffice:

``This paper presents work whose goal is to advance the field of Machine
Learning. There are many potential societal consequences of our work, none
which we feel must be specifically highlighted here.''

The above statement can be used verbatim in such cases, but we encourage
authors to think about whether there is content which does warrant further
discussion, as this statement will be apparent if the paper is later flagged
for ethics review.

% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite
\nocite{langley00}

==> sections/02_background.v0.tex <==
\section{Related Work}
\kk{You have 1.5 columns of related work in intro -- you definitely do not need more related work here.}
\textbf{Coding benchmarks.}
Since the emergence of LLMs, the application of LLMs to software engineering (SE) tasks has become ubiquitous.
%\petros{Well, that's not quite true. People have been doing MSR work since the 2010s, and it was pretty popular in ML. Perhaps "has reached impressively practical levels"?}
To evaluate LLMs, many benchmarks have been proposed for code generation (a crucial task in SE).
Early benchmarks such as HumanEval \cite{chen2021codex} and MBPP \cite{austin2021programsynthesislargelanguage} focused on self-contained function-level synthesis from docstrings.
Evolving from single-file editing tasks, SWE-bench \cite{jimenez2023swe} introduced repository-level bug resolution tasks in real-world code repositories. 
%As SWE-Bench was the first benchmark targeting code-generation at repository-scale, it is understandably focused and thus has many limitations. 
SWE-bench targets a single userspace language (Python), and has a cap on context size --- the maximum lines in a repository being under $1M$. Thus, subsequent works addressed some of these limitations \cite{deng2025swe}.
%\petros{(e.g., SWE-Bench Pro, Lancer, etc.)}.
Most recently, \citet{mathai2024kgym} introduced the challenging task of crash-resolution in large operating system codebases, such as the Linux kernel, by open-sourcing two challenging datasets (\data and \dataC). We build upon this latest work by identifying and addressing a key limitation noted below.

% pushed the frontier of complex code generation tasks by proposing more challenging Linux kernel bug fixing tasks in kBenchSyz and kBenchC.

The aforementioned benchmarks suffer from an important problem --- they do not automatically self-evolve as they largely involve manual curation. To partially address this issue, recent efforts harness automatic curation pipelines to (1) scale up SE instances to train LLMs \cite{yang2025swe, faircodegenteam2025cwmopenweightsllmresearch} and (2) provide %contamination-free 
fresh coding benchmarks \cite{zhang2025swe, jain2024livecodebench}. 
%and (2) they do not quantitatively measure the impact of data contamination on LLM efficacy. 
% \junfeng{this is more a study that we can conduct. focusing on the limitation of not self-evolving is enough I think.} 
% \alex{Noted}
%that the source data might have been included in LLM training.
% To partially address the second issue, some recent efforts harness automatic curation pipelines to (1) scale up SE instances to train LLMs \cite{yang2025swe, faircodegenteam2025cwmopenweightsllmresearch} and (2) provide contamination-free coding benchmarks \cite{zhang2025swe, jain2024livecodebench}. 
More specifically, \citet{jain2024livecodebench} evaluates LLMs on the latest competitive programming problems from LeetCode \cite{leetcode}, AtCoder \cite{atcoder}, and Codeforces \cite{codeforces};
%measuring LLM efficacy within a given time window.
while \citet{zhang2025swe} benchmarks coding agents with freshly curated SWE-bench tasks.
% Subsequently, \citet{zhang2025swe} benchmarked coding agents with freshly curated SWE-bench tasks in SWE-bench-Live \cite{zhang2025swe}.

% Proceeding from previous work, \lkbench evaluates coding agents and LLMs with freshly curated Linux kernel bugs from \syzbot, proposing more challenging tasks that have zero chance being included in LLMs training.

In alignment with previous works \cite{mathai2024kgym}, \lkbench also targets the problem of repository-level crash resolution for the Linux operating system. Different from previous works, \lkbench is (1) \emph{self-evolving}, as it continuously fetches freshly curated Linux kernel bugs from \syzbot \cite{syzbot}, and (2) \emph{time and attribute sensitive}, as it evaluates state-of-the-art agents on problems beyond the knowledge cut-off for various LLM vendors.
%\alex{What about SEC Bench ?}


\textbf{Agents.}

% Benchmarks consisting of repository-level tasks show primitive performance by packing all necessary information in a single-shot context \cite{mathai2024kgym, jimenez2023swe}.

% SWE-agent sets the new paradigm of autonomous software engineering agents equipped with computer-use tools \cite{yang2024swe}, and the bash-only mini-SWE-agent is used for the current SWE-bench evaluations on its website \cite{jimenez2023swe, swebenchleaderboards, yang2024swe}.
% Following agentic frameworks include OpenHands \cite{wang2024openhands}, TRAE \cite{traeresearchteam2025traeagent}, Live-SWE-agent \cite{xia2025live}.
% In this paper, we benchmark the representative coding agents in \cref{} and compare their performance on the Linux bugs fixing tasks. \chenxi{TODO}

Primitive agents that pack all necessary information into a single prompt have been shown to achieve abysmal performance on benchmarks consisting of repository-level tasks \citep{mathai2024kgym, jimenez2023swe}.
For example, \citep{mathai2024kgym} demonstrated that even when prompting LLMs with the exact oracle files, the crash resolution rate remained very low on the kBenchSyz dataset.
Recently, \swe \cite{yang2024swe} sets the new paradigm of autonomous SE agents by equipping LLMs with computer-use tools, and its bash-only scaffold variant (\mini) is currently used to evaluate various LLMs on the SWE-bench dataset \citep{jimenez2023swe, swebenchleaderboards, yang2024swe}. Subsequently, there were many follow-up agentic frameworks, including \oh \cite{wang2024openhands}, TRAE \cite{traeresearchteam2025traeagent}, \live \cite{xia2025live}, CodeResearcher \cite{singh2025code} and \cf \cite{mathai2025crashfixer}.
In this work, we benchmark the representative coding agents in \S\ref{sec:exp_agent} and compare their performance on Linux kernel crash-resolution tasks.

% \paragraph{kGym} In order to benchmark LLMs on Linux kernel crash resolution, kGym abstracts the heavy lifting of kernel compilation and reproducer testing in a distributed system \cite{mathai2024kgym}.
% However, before the emerging coding agents, Mathai et al. benchmarked LLMs on kBenchSyz with all-in-one prompts without agentic scaffolding.
% kGymSuite, a following iteration of kGym, was proposed to support CrashFixer for crash resolution feedback as well as final patch evaluation \cite{mathai2025crashfixer, huang2025kgymsuite}.
% The workflow-based agent CrashFixer was able to verify its current edit through kGymSuite during runtime \cite{mathai2025crashfixer}.
% In our work, we extended kGymSuite with \kenv to support crash resolution feedback and final patch evaluation for the representative agents, and this support can be easily extended to other agents.
% We evaluate the performance of current LLMs and agents in \cref{}. \chenxi{TODO}

\textbf{\kgym.} 
%\kenv connects each \compenv to \kgym \cite{mathai2024kgym}, 
\kgym \cite{mathai2024kgym} is an existing platform capable of running large-scale Linux kernel crash-resolution experiments. With a simple API, \kgym abstracts aways the heavy lifting of kernel compilation and execution in a distributed system. 
%As \kgym was built to support a simple API that takes a single bug patch, applies the patch to the codebase, compiles the kernel, and runs the reproducer, it is better 
% However, it is tailored towards one-shot prompting strategies. 
Subsequently, \kgymsuite \cite{kgymsuite} an improvement over \kgym
%\junfeng{it is code not paper but the way we cite it makes readers think that there's a paper} 
%\rayb{I agree, also as here you mentioned about it, it may not be required again and again to talk about \kgymsuite. We can just say \kenv } 
was open-sourced ---  faster, more scalable, and capable of supporting \cf, a workflow-based agent \cite{mathai2025crashfixer}. However, this solution was specific to \cf and not generalizable. Hence, we develop \kenv to provide a truly agent-agnostic \compenv. This \compenv is connected to \kgymsuite to provide agents with the needed support for compilation and execution. With {\kenv}'s \compenv, we show evaluations for three APR agents in \S\ref{sec:exp_agent}, highlighting its extensibility.
%by improving upon \kgymsuite and providing a truly \emph{agent-agnostic} execution environment that can provide (i) iterative crash-resolution feedback, and (ii) the required environment setup, including the appropriate repository, commit specification, anti-cheat guardrails, and all the required file-related support. 
% We evaluate the performance of several coding agents with the \kenv environment on \lkbench. We attest that the environment is truly extensible and easy to plug into many agents with bash-invoking capability.\junfeng{We attest -- read a bit weird. we have eval experiments to support this, no need to attest. just say we show in evaluation that it can support N very different agents}

In the following sections, we delve deeper into our major contributions --- \S\ref{sec:kenv} describes the internals of \kenv and how agents interact with our provided {\compenv}s; \S\ref{sec:live_kbench_sec} details the complete pipeline that supports self-evolving benchmarks, and finally \S\ref{sec:exp} depicts the interesting experiments and studies that one can perform when \lkbench and \kenv work seamlessly together.
